MetaSDF: Meta-learning Signed Distance Functions

Neural implicit shape representations are an emerging paradigm that offers many potential benefits over conventional discrete representations, including memory efficiency at a high spatial resolution. Generalizing across shapes with such neural implicit representations amounts to learning priors over the respective function space and enables geometry reconstruction from partial or noisy observations. Existing generalization methods rely on conditioning a neural network on a low-dimensional latent code that is either regressed by an encoder or jointly optimized in the auto-decoder framework. Here, we formalize learning of a shape space as a meta-learning problem and leverage gradient-based meta-learning algorithms to solve this task. We demonstrate that this approach performs on par with auto-decoder based approaches while being an order of magnitude faster at test-time inference. We further demonstrate that the proposed gradient-based method outperforms encoder-decoder based methods that leverage pooling-based set encoders.

==> sections/2D_experiments.tex <==
\subsection{Additional Results}
%
We provide mean and standard deviation for quantitative 2D SDF experiments for the conditional neural process and MetaSDF results in tables~\ref{tbl:2D_dense_vs_levelset_statistics} and ~\ref{tbl:2D_ood_statistics}.
%
In addition to the conditional neural process with a 4-layer ReLU set encoder, we report mean and standard deviation for a conditional neural process with a 9-layer ReLU set encoder. While the number of layers more than doubled, performance increases only slightly, still lagging far behind the performance of the proposed MetaSDF approach.
%
%Due to the time required for test set reconstruction in the auto-decoder framework, we do not report mean and standard deviation for the hypernetwork and concatenation-based approaches.


\begin{table}[h!]
\centering
\caption{$\ell_1$-error (mean/std.) for reconstructions from dense and levelset observations. All results are $\times 10^{-6}$. }
\label{tbl:2D_dense_vs_levelset_statistics}
	\begin{tabularx}{0.7\textwidth}{@{}lcccc@{}}
	        \toprule
	        & \phantom{} & Dense & \phantom{} & Zero-level set \\
	        \midrule
%			HyperNet && \num{50.449}/\num{0.263} && \num{1254.326}/\num{2.561} \\
%			Concat && \num{54.716}/\num{0.150} && \num{1859.307}/\num{3.764} \
	        Cond. NP, 4-layer set encoder && \num{101.7}/\num{5.1} && \num{154.9}/\num{1.0} \\
	        Cond. NP, 9-layer set encoder && \num{92.5}/\num{2.0} && \num{145.8}/\num{1.2} \\
	        MetaSDF && \textbf{15.4}/\textbf{0.2} && \textbf{56.6}/\textbf{0.5} \\
	        \bottomrule
	\end{tabularx}
\end{table}


\begin{table}[t!]
\centering
\caption{$\ell_1$-error (mean/std.) for reconstruction of out-of-distribution samples. All results are $\times 10^{-6}$. }
\label{tbl:2D_ood_statistics}
\begin{tabularx}{0.9\textwidth}{@{}lcccccc@{}}
        \toprule
        & \phantom{} & Unseen Digit & \phantom{} & Rotation & \phantom{} & Composit. \\
        \midrule
%        HyperNet && \num{70.363}/\num{0.245} && \num{150.374}/\num{0.115} && \num{227.830}/\num{3.018} \\
%	Concat && \num{48.284}/\num{0.120} && \num{143.995}/\num{0.048} && \num{127.316}/\num{0.689} \\
        Cond. NP, 4-layer set encoder && \num{252.4}/\num{5.0} && \num{301.1}/\num{10.3} && 484.9/13.6 \\
        Cond. NP, 9-layer set encoder && \num{223.4}/4.2 && \num{291.2}/8.6 && 468.0/22.8 \\
        MetaSDF && \textbf{22.8}/\textbf{0.5} && \textbf{33.3}/\textbf{1.1} && \textbf{59.8}/\textbf{1.2} \\
        \bottomrule
\end{tabularx}
\end{table}



\subsection{Reproducibility}
Here, we provide exact specifications of the 2D experiments to ensure reproducibility. All code and datasets will be made publicly available.

\subsubsection{Datasets}
%
For all single-MNIST experiments, we use the MNIST dataset, as supplied with the pytorch torchvision library (\href{https://pytorch.org/docs/stable/torchvision/datasets.html}{link}), as a starting point.
%
We use the official train-test split of the MNIST dataset, and further split 1000 examples off the training set as a validation set.
%
For the double-MNIST and triple-MNIST experiments, we use the datasets provided by~\cite{mulitdigitmnist} (\href{https://github.com/shaohua0116/MultiDigitMNIST}{link}).
%
The large size of the triple-MNIST test set makes it infeasible to reconstruct it using the auto-decoder framework. We thus only pick 1000 elements of the triple-MNIST dataset as a test set.
%
To extract 2D signed distance functions, we first binarize the greyscale image, and then apply two unsigned 2D distance transforms as implemented in the scipy package, once on the original binary image and once on its inverse binary image, and combine them into a single signed distance function.

\subsubsection{Model Details}
%
All models are implemented as fully connected ReLU-MLPs with $256$ hidden units and no normalization layers.
%
The SDF network $\Phi$ is implemented with four layers (i.e., two hidden layers).
%
The concatenation-based conditioning is performed by concatenating the latent code once to the input and once to the third layer of $\Phi$.
%
The set encoder of CNPs is implemented with four layers. Hypernetworks are implemented with three layers as in~\cite{sitzmann2019srns}, predicting all parameters (weights and biases) of $\Phi$.
%
The proposed approach performs $5$ inner-loop update steps, where we initialize $\alpha$ as \num{1e-1}.
%

\subsubsection{Out-of-distribution experiments}
%
We conduct all out-of-distribution experiments using models trained on \emph{dense} samples from the signed distance function, and condition on dense samples at test-time as well. We note that baseline approaches performed much better in the dense setting, and this thus enables the fairest comparison of the proposed approach and baseline approaches. 

\subsubsection{Hyperparameters}
%
We train all models with ADAM with a learning rate of \num{1e-4} and a batch size of 32, sampling $32^2$ points for the dense SDF experiments and $512$ points for the levelset experiments. 
%
We train encoder- and meta-learning based models for 50 epochs. Due to slower convergence of the auto-decoder framework, we train auto-decoder models for 150 epochs.

\subsubsection{Computing Hardware}
%
We train all models on a single NVIDIA RTX 6000 GPU.
%
Hypernetworks, conditioning via concatenation-based models, as well as conditional neural processes consume approximately 3GB of GPU memory at training time.
%
The proposed MetaSDF approach consumes approximately 5GB of GPU memory at training time.

\subsubsection{Runtime \& Complexity}
%
Conditional neural processes train in about 3 hours, while MetaSDF trains in about 5 hours.
%
The training time of auto-decoder based approaches grows significantly with the size of the dataset. For out-of-distribution experiments such as the rotated MNIST digits or the compositionality experiments, the size of the datasets required 24 hours of training per model, and another 24 hours of test-time reconstruction. 
%
The memory complexity of the proposed Meta-Learning approach is $O(nm)$, with the number of query points $n$ and the number of inner gradient descent steps $m$.

\subsubsection{Number of Evaluation Runs}
%
Each method was run on the test set exactly three times to calculate mean and standard deviation of the final result.

==> sections/3D_experiments.tex <==
\subsection{Additional Results}

\subsubsection{``Average airplane'' of concatenation-based approach vs. Meta-network initialization}
%
\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.5\textwidth]{supplement_figures/supplement_metasdf_vs_deepsdf_mean}
	\caption{Comparison of the zero-level set of MetaSDF before specialization and the ``mean plane'' of DeepSDF, i.e., the zero-level set of the airplane encoded by the all-zero latent code.}
	\label{fig:initialization}
\end{figure*}

In Fig.~\ref{fig:initialization}, we show the zero-level set of the meta-initialization discovered by the proposed MetaSDF approach as well as the zero-level set of the SDF corresponding to the all-zero ``mean latent code'' as discovered by DeepSDF~\cite{park2019deepsdf}.
%
Intriguingly, they bear little resemblance. Future work may investigate the properties of the initialization of MetaSDF, potentially providing insight into why this initialization enables such swift specialization with only five gradient descent steps.

\subsubsection{Qualitative comparison to DeepSDF and PointNet encoder on Shapenet V2 Tables}
Fig.~\ref{fig:qual_deepsdf_tables} and Fig.~\ref{fig:qual_pointnet_tables} show qualitative comparisons of the proposed MetaSDF approach to DeepSDF and a pointnet-encoder based approach on the Shapenet V2 tables class.

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{supplement_figures/tables_gt_deepsdf_metasdf}
	\caption{Qualitative comparison of the proposed MetaSDF approach and DeepSDF on the Shapenet v2 tables dataset.}
	\label{fig:qual_deepsdf_tables}
\end{figure*}

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{supplement_figures/tables_gt_onet_metasdf}
	\caption{Qualitative comparison of the proposed MetaSDF approach and a PointNet Encoder on zero-level set reconstructions from the Shapenet v2 tables dataset.}
	\label{fig:qual_pointnet_tables}
\end{figure*}

\subsection{Reproducibility.}
Here, we provide exact specifications of the 3D experiments to ensure reproducibility. All code and datasets will be made publicly available.

\subsubsection{Datasets.}
We utilize the 'Planes' and 'Tables'  categories of ShapeNetV2~\cite{chang2015shapenet} (\href{https://www.shapenet.org/}{link}) for all 3D experiments. We preprocess SDF samples, used in dense reconstruction, and surface samples, used in zero-level set reconstruction, with the preprocessing code (\href{https://github.com/facebookresearch/DeepSDF}{link}) from DeepSDF~\cite{park2019deepsdf}. We use DeepSDF's train-test splits for both object categories, but extract 20 examples from each training set for use as validation sets. We encountered errors in using DeepSDF's preprocessing code and thus were only able to process about 80\% of the 3D models. 

\subsubsection{Model Details.}
\paragraph{Details on composite loss}
Empirically, we found that a composite loss function that combines the $\ell_1$ loss on the value of the predicted SDF with a binary crossentropy loss on the sign of the predicted SDF lead to better results for MetaSDF. Because meshes are represented by the zero-level set, precisely predicting the sign of the SDF close to the surface is far more important to mesh accuracy than accurately predicting the value of the SDF away from the surface. Intuitively, our strategy encourages the model to emphasize not only the value but also the sign of SDF predictions. Our model predicts two outputs: a prediction of signed distance and a sigmoid output representing the sign. At training time, we calculate the $\ell_1$ loss on the SDF prediction and the binary crossentropy loss on the sign prediction. We combine these loss terms with the method proposed by Kendall et al.~\cite{kendall2018multi}.  At test time, we combine the two outputs by multiplying the absolute value of the distance prediction with the predicted sign to produce a single SDF prediction.

\paragraph{Dense MetaSDF}
MetaSDF for our dense experiments is implemented as a fully connected ReLU-MLP with 8 layers of 512 units and no normalization layers. We utilize 5 inner-loop update steps and per-parameter, per-step learning rates, which are initialized to \num{5e-3}.

\paragraph{Zero-Level set MetaSDF}
We utilize a similar architecture for our zero-level set experiments, but in order to better match parameter counts to PointNet encoders, we reduced network size to 7 layers of 512 units.

\paragraph{DeepSDF}
We utilize the official DeepSDF implementation, which consists of 8 layers of 512 units and weight normalization. DeepSDF uses an autodecoder, with latent codes of 256 units.

\paragraph{PointNet Encoder}
We implement a resnet PointNet encoder, which consists of 5 resnet blocks of 512 units and encodes a 256-dimensional latent code. The SDF network, $\Phi$ , is implemented with 7 layers of 512 units.

\subsubsection{Hyperparameters.}
We train all models with ADAM and initialize learning rates to \num{5e-4}. All models were trained to convergence. We trained Dense MetaSDF for 500 epochs using our composite loss function and decayed learning rate by a factor of 0.5 after 350 steps. All other models, including Zero-level set MetaSDF, were trained using L1 loss for 2000 epochs, decaying learning rate by a factor of 0.5 every 500 steps. All models use a batch size of 64 scenes.

\subsubsection{Computing Hardware}
%
We train all models on dual NVIDIA RTX 8000 GPUs.

\subsubsection{Runtime \& Complexity.}
The complexity of the proposed Meta-Learning approach is $O(nm)$, with the number of query points $n$ and the number of inner gradient descent steps $m$. DeepSDF and PointNet Encoders train to 2000 epochs in approximately 4 days while MetaSDF trains to 2000 epochs in approximately 6 days.

\subsubsection{Number of Evaluation Runs.}
Because we randomly sample context points during mesh reconstruction, reconstructed meshes vary between runs. Following the evaluation procedure of DeepSDF, at test-time each model reconstructs each mesh twice; the better reconstruction is used in computing chamfer distance across the test set. This evaluation procedure was conducted once for each model.


